Automated Creation of Digital Cousins for Robust Policy Learning

Training robot policies in the real world can be unsafe, costly, and difficult to scale. Simulation serves as an inexpensive and potentially limitless source of training data, but suffers from the semantics and physics disparity between simulated and real-world environments. These discrepancies can be minimized by training in digital twins, which serve as virtual replicas of a real scene but are expensive to generate and cannot produce cross-domain generalization. To address these limitations, we propose the concept of digital cousins, a virtual asset or scene that, unlike a digital twin, does not explicitly model a real-world counterpart but still exhibits similar geometric and semantic affordances. As a result, digital cousins simultaneously reduce the cost of generating an analogous virtual environment while also facilitating better robustness during sim-to-real domain transfer by providing a distribution of similar training scenes. Leveraging digital cousins, we introduce a novel method for their automated creation, and propose a fully automated real-to-sim-to-real pipeline for generating fully interactive scenes and training robot policies that can be deployed zero-shot in the original scene. We find that digital cousin scenes that preserve geometric and semantic affordances can be produced automatically, and can be used to train policies that outperform policies trained on digital twins, achieving 90% vs. 25% success rates under zero-shot sim-to-real transfer. Additional details are available at https://digital-cousins.github.io/.

==> figs/sim2sim_ablation_fig.tex <==
% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=\textwidth]{figs/sim2sim_fig_interpolate.pdf}
%     \caption{Qualitative results of our ACDC pipeline on the sim-to-sim setting. In each row, the left image is the single input RGB image to our ACDC pipeline with background semi-transparent, and the right three images are visualization of our reconstructed scene from three different view points.}
%     \label{fig:sim2sim}
% \end{figure}

\begin{figure}[h!]
    \centering
    \includegraphics[width=\textwidth]{figs/figs/sim2sim_figure_6fig.pdf}
    \caption{Qualitative results of our ACDC pipeline on the sim-to-sim setting. The upper row shows the single input RGB image to ACDC, while the second row shows the corresponding reconstructed scene.}
    \label{fig:sim2sim}
\end{figure}

==> table/sim2sim.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \resizebox{0.99\textwidth}{!}{%
    \begin{tabular}{ccccccccc}
    Input Scene & \acdc Output & Scale (m) &  & Cat. & Mod. & L2 Dist (cm) $\downarrow$ & Ori. Diff. $\downarrow$ & Bbox IoU $\uparrow$ \\
    \midrule
     \multirow{4}[1]{*}{\includegraphics[width=2.5cm]{figs/figs/sim2sim_reconstruction/DiningRoom_interpolated.png}} & \multirow{4}[1]{*}{\includegraphics[width=2.5cm]{figs/figs/sim2sim_reconstruction/DiningRoom_out.png}} & \multirow{4}[2]{*}{3.42} & (a)   & \multirow{2}[1]{*}{6/6} & \multirow{2}[1]{*}{4/6} & \textbf{4.79 ± 1.52} & \textbf{0.07 ± 0.03} & 0.54 ± 0.32 \\
    &   &    & (b)   &       &       & 4.85 ± 1.52 & 0.08 ± 0.01 & 0.54 ± 0.32 \\
    \cmidrule{8-8}
    &    &   & (c)   & \multirow{2}[1]{*}{6/6} & \multirow{2}[1]{*}{\textbf{6/6}} & 4.87 ± 1.83 & 0.12 ± 0.13 & 0.54 ± 0.31 \\
    &   &    & (d)   &       &       & 5.03 ± 1.53 & \textbf{0.10 ± 0.11} & 0.54 ± 0.32  \\
    \midrule
    \multirow{4}[1]{*}{\includegraphics[width=2.5cm]{figs/figs/sim2sim_reconstruction/living_room2_interpolated.png}} & \multirow{4}[1]{*}{\includegraphics[width=2.5cm]{figs/figs/sim2sim_reconstruction/living_room2_out.png}} & \multirow{4}[2]{*}{4.17} & (a)   & \multirow{2}[1]{*}{8/8} & \multirow{2}[1]{*}{3/8} & \textbf{7.81 ± 4.87} & 0.05 ± 0.00 & 0.65 ± 0.18\\
    &    &   & (b)   &       &       & 7.91 ± 5.04 & 0.05 ± 0.00 & 0.65 ± 0.19 \\
    \cmidrule{8-8}
    &   &    & (c)   & \multirow{2}[1]{*}{8/8} & \multirow{2}[1]{*}{\textbf{6/8}} & 7.94 ± 5.01 & 0.05 ± 0.00 & \textbf{0.66 ± 0.17}  \\
    &   &    & (d)   &       &       & 7.94 ± 5.01 & 0.05 ± 0.00 & \textbf{0.66 ± 0.17} \\
    \midrule
    \multirow{4}[1]{*}{\includegraphics[width=2.5cm]{figs/figs/sim2sim_reconstruction/recreation_room_interpolated.png}} & \multirow{4}[1]{*}{\includegraphics[width=2.5cm]{figs/figs/sim2sim_reconstruction/recreation_room_out.png}} & \multirow{4}[1]{*}{6.89} & (a)   & \multirow{2}[1]{*}{12/12} & \multirow{2}[1]{*}{6/12} & 7.27 ± 5.51 & 0.46 ± 0.50 & 0.54 ± 0.30  \\
    &   &    & (b)   &       &       & 6.31 ± 4.78 & \textbf{0.24 ± 0.49} & 0.64 ± 0.26 \\
    \cmidrule{8-8}
    &   &    & (c)   & \multirow{2}[0]{*}{12/12} & \multirow{2}[0]{*}{\textbf{11/12}} & \textbf{6.15 ± 4.50} & 0.25 ± 0.47 & 0.67 ± 0.22   \\
    &   &    & (d)   &       &       & 5.96 ± 4.35 & \textbf{0.05 ± 0.04} & \textbf{0.70 ± 0.18} \\
    \midrule
    \multirow{4}[0]{*}{\includegraphics[width=2.5cm]{figs/figs/sim2sim_reconstruction/gym_interpolated.png}} & \multirow{4}[0]{*}{\includegraphics[width=2.5cm]{figs/figs/sim2sim_reconstruction/gym_out.png}} & \multirow{4}[0]{*}{10.23} & (a)   & \multirow{2}[0]{*}{15/15} & \multirow{2}[0]{*}{12/15} & 17.40 ± 9.05 & 0.17 ± 0.17 & 0.49 ± 0.20 \\
    &   &    & (b)   &       &       & \textbf{17.01 ± 9.34} & \textbf{0.15 ± 0.14} & 0.51 ± 0.20  \\
    \cmidrule{8-8}
    &   &    & (c)   & \multirow{2}[0]{*}{15/15} & \multirow{2}[0]{*}{\textbf{15/15}} & 17.16 ± 9.31 & 0.16 ± 0.17 & 0.51 ± 0.22 \\
    &   &    & (d)   &       &       & 17.09 ± 9.26 & \textbf{0.11 ± 0.10} & \textbf{0.55 ± 0.21}  \\
    \midrule
    \end{tabular}%
  }
  \caption{Quantitative and qualitative evaluation of scene reconstruction using our ACDC method in a sim-to-sim scenario. `Scale' is the largest distance between two objects' bounding boxes in the input scene. `Cat.' indicates the ratio of correctly categorized objects to the total number of objects in the scene. `Mod.' shows the ratio of correctly modeled objects to the total number of objects in the scene. `L2 Dist' provides the mean and standard deviation of the Euclidean distance between the centers of the bounding boxes in the input and reconstructed scenes. `Ori. Diff.' represents the mean and standard deviation of the orientation magnitude difference of each non-uniformly symmetric object. `Bbox IoU' presents the Intersection over Union (IoU) for assets' 3D bounding boxes. Please refer to the supplementary material for extension of this table.\label{tab:sim2sim}}
\end{table}%


==> table/sim2sim_full_table.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \begin{adjustwidth}{-1.5cm}{}
    \begin{tabular}{cccccccccc}
    Input Scene & \acdc Output & Scale (m) &  & Cat. & Mod. & L2 Dist (cm) $\downarrow$ & Ori. Diff. $\downarrow$ & Bbox IoU $\uparrow$ & Ori. Bbox IoU $\uparrow$  \\
    \midrule
    \multirow{4}[1]{*}{\includegraphics[width=2.5cm]{figs/figs/sim2sim_reconstruction/bathroom_interpolated.png}} & \multirow{4}[1]{*}{\includegraphics[width=2.5cm]{figs/figs/sim2sim_reconstruction/bathroom_out.png}} & \multirow{4}[2]{*}{3.68} & (a)   & \multirow{2}[1]{*}{5/5} & \multirow{2}[1]{*}{5/5} & 5.27 ± 2.85 & 0.07 ± 0.07 & 0.75 ± 0.14 & 0.64 ± 0.07  \\
    &   &    & (b)   &       &       & 5.27 ± 2.85 & 0.07 ± 0.07 & 0.75 ± 0.14 & 0.64 ± 0.07 \\
    &   &    & (c)   & \multirow{2}[1]{*}{5/5} & \multirow{2}[1]{*}{5/5} & 5.27 ± 2.85 & 0.07 ± 0.07 & 0.75 ± 0.14 & 0.64 ± 0.07 \\
    &   &    & (d)   &       &       & 5.27 ± 2.85 & 0.07 ± 0.07 & 0.75 ± 0.14 & 0.64 ± 0.07 \\
    \midrule
     \multirow{4}[1]{*}{\includegraphics[width=2.5cm]{figs/figs/sim2sim_reconstruction/DiningRoom_interpolated.png}} & \multirow{4}[1]{*}{\includegraphics[width=2.5cm]{figs/figs/sim2sim_reconstruction/DiningRoom_out.png}} & \multirow{4}[2]{*}{3.42} & (a)   & \multirow{2}[1]{*}{6/6} & \multirow{2}[1]{*}{4/6} & \textbf{4.79 ± 1.52} & \textbf{0.07 ± 0.03} & 0.54 ± 0.32 & 0.52 ± 0.28 \\
    &   &    & (b)   &       &       & 4.85 ± 1.52 & 0.08 ± 0.01 & 0.54 ± 0.32 & 0.52 ± 0.28 \\
    \cmidrule{7-7}
    &    &   & (c)   & \multirow{2}[1]{*}{6/6} & \multirow{2}[1]{*}{\textbf{6/6}} & 4.87 ± 1.83 & 0.12 ± 0.13 & 0.54 ± 0.31 & 0.53 ± 0.28 \\
    &   &    & (d)   &       &       & 5.03 ± 1.53 & \textbf{0.10 ± 0.11} & 0.54 ± 0.32 & 0.52 ± 0.29  \\
    \midrule
    \multirow{4}[1]{*}{\includegraphics[width=2.5cm]{figs/figs/sim2sim_reconstruction/LivingRoom1_interpolated.png}} & \multirow{4}[1]{*}{\includegraphics[width=2.5cm]{figs/figs/sim2sim_reconstruction/LivingRoom1_out.png}} & \multirow{4}[2]{*}{2.91} & (a)   & \multirow{2}[1]{*}{6/6} & \multirow{2}[1]{*}{4/6} & \textbf{5.51 ± 2.71} & 0.03 ± 0.00 & 0.64 ± 0.16 & \textbf{0.60 ± 0.17} \\
    &    &   & (b)   &       &       & 5.97 ± 2.56 & 0.03 ± 0.00 & 0.64 ± 0.16 & \textbf{0.60 ± 0.17} \\
    \cmidrule{7-7}
    &   &    & (c)   & \multirow{2}[1]{*}{6/6} & \multirow{2}[1]{*}{\textbf{5/6}} & 7.13 ± 4.77 & 0.16 ± 0.19 & 0.54 ± 0.24 & 0.51 ± 0.21  \\
    &   &    & (d)   &       &       & 5.60 ± 2.92 & \textbf{0.10 ± 0.10} & \textbf{0.65 ± 0.18} & \textbf{0.60 ± 0.17}  \\
    \midrule
    \multirow{4}[1]{*}{\includegraphics[width=2.5cm]{figs/figs/sim2sim_reconstruction/bedroom_interpolated.png}} & \multirow{4}[1]{*}{\includegraphics[width=2.5cm]{figs/figs/sim2sim_reconstruction/bedroom_out.png}} & \multirow{4}[1]{*}{3.54} & (a)   & \multirow{2}[1]{*}{5/5} & \multirow{2}[1]{*}{2/5} & \textbf{6.47 ± 2.79} & 0.04 ± 0.01 & \textbf{0.64 ± 0.23} & \textbf{0.65 ± 0.28}  \\
    &    &   & (b)   &       &       & 6.83 ± 3.20 & \textbf{0.03 ± 0.01} & 0.63 ± 0.24 & 0.64 ± 0.30  \\
    \cmidrule{7-7}
    &   &    & (c)   & \multirow{2}[0]{*}{5/5} & \multirow{2}[0]{*}{\textbf{3/5}} & 6.51 ± 2.77 & 0.03 ± 0.01 & \textbf{0.64 ± 0.22} & 0.60 ± 0.20 \\
    &   &    & (d)   &       &       & 6.90 ± 3.21 & 0.03 ± 0.01 & 0.62 ± 0.24 & 0.58 ± 0.22 \\
    \midrule
    \multirow{4}[1]{*}{\includegraphics[width=2.5cm]{figs/figs/sim2sim_reconstruction/kitchen_interpolated.png}} & \multirow{4}[1]{*}{\includegraphics[width=2.5cm]{figs/figs/sim2sim_reconstruction/kitchen_out.png}}  & \multirow{4}[1]{*}{3.24} & (a)   & \multirow{2}[0]{*}{5/6} & \multirow{2}[0]{*}{3/6} & 6.64 ± 3.34 & 0.24 ± 0.20 & 0.57 ± 0.21 & 0.58 ± 0.15 \\
    &   &    & (b)   &       &       & 5.92 ± 3.32 & \textbf{0.06 ± 0.03} & \textbf{0.69 ± 0.14} & 0.66 ± 0.14  \\
    \cmidrule{7-7}
    &   &    & (c)   & \multirow{2}[1]{*}{5/6} & \multirow{2}[1]{*}{\textbf{5/6}} & 6.00 ± 3.79 & 0.06 ± 0.05 & 0.68 ± 0.14 & 0.65 ± 0.14 \\
    &   &    & (d)   &       &       & \textbf{5.33 ± 3.77} & \textbf{0.04 ± 0.03} & \textbf{0.69 ± 0.15} & \textbf{0.67 ± 0.15} \\
    \midrule
    \multirow{4}[1]{*}{\includegraphics[width=2.5cm]{figs/figs/sim2sim_reconstruction/living_room2_interpolated.png}} & \multirow{4}[1]{*}{\includegraphics[width=2.5cm]{figs/figs/sim2sim_reconstruction/living_room2_out.png}} & \multirow{4}[2]{*}{4.17} & (a)   & \multirow{2}[1]{*}{8/8} & \multirow{2}[1]{*}{3/8} & \textbf{7.81 ± 4.87} & 0.05 ± 0.00 & 0.65 ± 0.18 & \textbf{0.64 ± 0.17}  \\
    &    &   & (b)   &       &       & 7.91 ± 5.04 & 0.05 ± 0.00 & 0.65 ± 0.19 & \textbf{0.64 ± 0.16}  \\
    \cmidrule{7-7}
    &   &    & (c)   & \multirow{2}[1]{*}{8/8} & \multirow{2}[1]{*}{\textbf{6/8}} & 7.94 ± 5.01 & 0.05 ± 0.00 & \textbf{0.66 ± 0.17} & 0.63 ± 0.17  \\
    &   &    & (d)   &       &       & 7.94 ± 5.01 & 0.05 ± 0.00 & \textbf{0.66 ± 0.17} & 0.63 ± 0.17 \\
    \midrule
    \multirow{4}[1]{*}{\includegraphics[width=2.5cm]{figs/figs/sim2sim_reconstruction/recreation_room_interpolated.png}} & \multirow{4}[1]{*}{\includegraphics[width=2.5cm]{figs/figs/sim2sim_reconstruction/recreation_room_out.png}} & \multirow{4}[1]{*}{6.89} & (a)   & \multirow{2}[1]{*}{12/12} & \multirow{2}[1]{*}{6/12} & 7.27 ± 5.51 & 0.46 ± 0.50 & 0.54 ± 0.30 & 0.55 ± 0.25 \\
    &   &    & (b)   &       &       & 6.31 ± 4.78 & \textbf{0.24 ± 0.49} & 0.64 ± 0.26 & 0.62 ± 0.25 \\
    \cmidrule{7-7}
    &   &    & (c)   & \multirow{2}[0]{*}{12/12} & \multirow{2}[0]{*}{\textbf{11/12}} & \textbf{6.15 ± 4.50} & 0.25 ± 0.47 & 0.67 ± 0.22 & 0.62 ± 0.20  \\
    &   &    & (d)   &       &       & 5.96 ± 4.35 & \textbf{0.05 ± 0.04} & \textbf{0.70 ± 0.18} & \textbf{0.63 ± 0.18}  \\
    \midrule
    \multirow{4}[0]{*}{\includegraphics[width=2.5cm]{figs/figs/sim2sim_reconstruction/gym_interpolated.png}} & \multirow{4}[0]{*}{\includegraphics[width=2.5cm]{figs/figs/sim2sim_reconstruction/gym_out.png}} & \multirow{4}[0]{*}{10.23} & (a)   & \multirow{2}[0]{*}{15/15} & \multirow{2}[0]{*}{12/15} & 17.40 ± 9.05 & 0.17 ± 0.17 & 0.49 ± 0.20 & 0.50 ± 0.19 \\
    &   &    & (b)   &       &       & \textbf{17.01 ± 9.34} & \textbf{0.15 ± 0.14} & 0.51 ± 0.20 & 0.50 ± 0.20  \\
    \cmidrule{7-7}
    &   &    & (c)   & \multirow{2}[0]{*}{15/15} & \multirow{2}[0]{*}{\textbf{15/15}} & 17.16 ± 9.31 & 0.16 ± 0.17 & 0.51 ± 0.22 & 0.51 ± 0.21  \\
    &   &    & (d)   &       &       & 17.09 ± 9.26 & \textbf{0.11 ± 0.10} & \textbf{0.55 ± 0.21} & \textbf{0.53 ± 0.21}  \\
    \midrule
    \end{tabular}%
  \end{adjustwidth}
  \caption{Quantitative evaluation of scene reconstruction using our ACDC method in a sim-to-sim scenario. `Cat.' indicates the ratio of correctly categorized objects to the total number of objects in the scene. 'Mod.' shows the ratio of correctly modeled objects to the total number of objects in the scene. 'L2 Dist' provides the mean and standard deviation of the Euclidean distance between the centers of the bounding boxes in the input and reconstructed scenes. 'Ori. Diff.' represents the mean and standard deviation of the orientation magnitude difference of each non-uniformly symmetric object. 'Bbox IoU' presents the Intersection over Union (IoU) for axis-aligned 3D bounding boxes. 'Ori. Bbox IoU' displays the IoU for oriented 3D bounding boxes.\label{tab:sim2sim}}
\end{table}%


==> table/sim2sim_table_less_column.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \begin{adjustwidth}{-1.5cm}{}
    \begin{tabular}{ccccccccc}
    Input Scene & \acdc Output & Scale (m) &  & Cat. & Mod. & L2 Dist (cm) $\downarrow$ & Ori. Diff. $\downarrow$ & Bbox IoU $\uparrow$ \\
    \midrule
    \multirow{4}[1]{*}{\includegraphics[width=2.5cm]{figs/figs/sim2sim_reconstruction/bathroom_interpolated.png}} & \multirow{4}[1]{*}{\includegraphics[width=2.5cm]{figs/figs/sim2sim_reconstruction/bathroom_out.png}} & \multirow{4}[2]{*}{3.68} & (a)   & \multirow{2}[1]{*}{5/5} & \multirow{2}[1]{*}{5/5} & 5.27 ± 2.85 & 0.07 ± 0.07 & 0.75 ± 0.14\\
    &   &    & (b)   &       &       & 5.27 ± 2.85 & 0.07 ± 0.07 & 0.75 ± 0.14  \\
    &   &    & (c)   & \multirow{2}[1]{*}{5/5} & \multirow{2}[1]{*}{5/5} & 5.27 ± 2.85 & 0.07 ± 0.07 & 0.75 ± 0.14 \\
    &   &    & (d)   &       &       & 5.27 ± 2.85 & 0.07 ± 0.07 & 0.75 ± 0.14 \\
    \midrule
     \multirow{4}[1]{*}{\includegraphics[width=2.5cm]{figs/figs/sim2sim_reconstruction/DiningRoom_interpolated.png}} & \multirow{4}[1]{*}{\includegraphics[width=2.5cm]{figs/figs/sim2sim_reconstruction/DiningRoom_out.png}} & \multirow{4}[2]{*}{3.42} & (a)   & \multirow{2}[1]{*}{6/6} & \multirow{2}[1]{*}{4/6} & \textbf{4.79 ± 1.52} & \textbf{0.07 ± 0.03} & 0.54 ± 0.32 \\
    &   &    & (b)   &       &       & 4.85 ± 1.52 & 0.08 ± 0.01 & 0.54 ± 0.32 \\
    \cmidrule{7-7}
    &    &   & (c)   & \multirow{2}[1]{*}{6/6} & \multirow{2}[1]{*}{\textbf{6/6}} & 4.87 ± 1.83 & 0.12 ± 0.13 & 0.54 ± 0.31 \\
    &   &    & (d)   &       &       & 5.03 ± 1.53 & \textbf{0.10 ± 0.11} & 0.54 ± 0.32  \\
    \midrule
    \multirow{4}[1]{*}{\includegraphics[width=2.5cm]{figs/figs/sim2sim_reconstruction/LivingRoom1_interpolated.png}} & \multirow{4}[1]{*}{\includegraphics[width=2.5cm]{figs/figs/sim2sim_reconstruction/LivingRoom1_out.png}} & \multirow{4}[2]{*}{2.91} & (a)   & \multirow{2}[1]{*}{6/6} & \multirow{2}[1]{*}{4/6} & \textbf{5.51 ± 2.71} & 0.03 ± 0.00 & 0.64 ± 0.16\\
    &    &   & (b)   &       &       & 5.97 ± 2.56 & 0.03 ± 0.00 & 0.64 ± 0.16 \\
    \cmidrule{7-7}
    &   &    & (c)   & \multirow{2}[1]{*}{6/6} & \multirow{2}[1]{*}{\textbf{5/6}} & 7.13 ± 4.77 & 0.16 ± 0.19 & 0.54 ± 0.24 \\
    &   &    & (d)   &       &       & 5.60 ± 2.92 & \textbf{0.10 ± 0.10} & \textbf{0.65 ± 0.18}\\
    \midrule
    \multirow{4}[1]{*}{\includegraphics[width=2.5cm]{figs/figs/sim2sim_reconstruction/bedroom_interpolated.png}} & \multirow{4}[1]{*}{\includegraphics[width=2.5cm]{figs/figs/sim2sim_reconstruction/bedroom_out.png}} & \multirow{4}[1]{*}{3.54} & (a)   & \multirow{2}[1]{*}{5/5} & \multirow{2}[1]{*}{2/5} & \textbf{6.47 ± 2.79} & 0.04 ± 0.01 & \textbf{0.64 ± 0.23} \\
    &    &   & (b)   &       &       & 6.83 ± 3.20 & \textbf{0.03 ± 0.01} & 0.63 ± 0.24  \\
    \cmidrule{7-7}
    &   &    & (c)   & \multirow{2}[0]{*}{5/5} & \multirow{2}[0]{*}{\textbf{3/5}} & 6.51 ± 2.77 & 0.03 ± 0.01 & \textbf{0.64 ± 0.22} \\
    &   &    & (d)   &       &       & 6.90 ± 3.21 & 0.03 ± 0.01 & 0.62 ± 0.24 \\
    \midrule
    \multirow{4}[1]{*}{\includegraphics[width=2.5cm]{figs/figs/sim2sim_reconstruction/kitchen_interpolated.png}} & \multirow{4}[1]{*}{\includegraphics[width=2.5cm]{figs/figs/sim2sim_reconstruction/kitchen_out.png}}  & \multirow{4}[1]{*}{3.24} & (a)   & \multirow{2}[0]{*}{5/6} & \multirow{2}[0]{*}{3/6} & 6.64 ± 3.34 & 0.24 ± 0.20 & 0.57 ± 0.21  \\
    &   &    & (b)   &       &       & 5.92 ± 3.32 & \textbf{0.06 ± 0.03} & \textbf{0.69 ± 0.14}  \\
    \cmidrule{7-7}
    &   &    & (c)   & \multirow{2}[1]{*}{5/6} & \multirow{2}[1]{*}{\textbf{5/6}} & 6.00 ± 3.79 & 0.06 ± 0.05 & 0.68 ± 0.14 \\
    &   &    & (d)   &       &       & \textbf{5.33 ± 3.77} & \textbf{0.04 ± 0.03} & \textbf{0.69 ± 0.15}  \\
    \midrule
    \multirow{4}[1]{*}{\includegraphics[width=2.5cm]{figs/figs/sim2sim_reconstruction/living_room2_interpolated.png}} & \multirow{4}[1]{*}{\includegraphics[width=2.5cm]{figs/figs/sim2sim_reconstruction/living_room2_out.png}} & \multirow{4}[2]{*}{4.17} & (a)   & \multirow{2}[1]{*}{8/8} & \multirow{2}[1]{*}{3/8} & \textbf{7.81 ± 4.87} & 0.05 ± 0.00 & 0.65 ± 0.18\\
    &    &   & (b)   &       &       & 7.91 ± 5.04 & 0.05 ± 0.00 & 0.65 ± 0.19 \\
    \cmidrule{7-7}
    &   &    & (c)   & \multirow{2}[1]{*}{8/8} & \multirow{2}[1]{*}{\textbf{6/8}} & 7.94 ± 5.01 & 0.05 ± 0.00 & \textbf{0.66 ± 0.17}  \\
    &   &    & (d)   &       &       & 7.94 ± 5.01 & 0.05 ± 0.00 & \textbf{0.66 ± 0.17} \\
    \midrule
    \multirow{4}[1]{*}{\includegraphics[width=2.5cm]{figs/figs/sim2sim_reconstruction/recreation_room_interpolated.png}} & \multirow{4}[1]{*}{\includegraphics[width=2.5cm]{figs/figs/sim2sim_reconstruction/recreation_room_out.png}} & \multirow{4}[1]{*}{6.89} & (a)   & \multirow{2}[1]{*}{12/12} & \multirow{2}[1]{*}{6/12} & 7.27 ± 5.51 & 0.46 ± 0.50 & 0.54 ± 0.30  \\
    &   &    & (b)   &       &       & 6.31 ± 4.78 & \textbf{0.24 ± 0.49} & 0.64 ± 0.26 \\
    \cmidrule{7-7}
    &   &    & (c)   & \multirow{2}[0]{*}{12/12} & \multirow{2}[0]{*}{\textbf{11/12}} & \textbf{6.15 ± 4.50} & 0.25 ± 0.47 & 0.67 ± 0.22   \\
    &   &    & (d)   &       &       & 5.96 ± 4.35 & \textbf{0.05 ± 0.04} & \textbf{0.70 ± 0.18} \\
    \midrule
    \multirow{4}[0]{*}{\includegraphics[width=2.5cm]{figs/figs/sim2sim_reconstruction/gym_interpolated.png}} & \multirow{4}[0]{*}{\includegraphics[width=2.5cm]{figs/figs/sim2sim_reconstruction/gym_out.png}} & \multirow{4}[0]{*}{10.23} & (a)   & \multirow{2}[0]{*}{15/15} & \multirow{2}[0]{*}{12/15} & 17.40 ± 9.05 & 0.17 ± 0.17 & 0.49 ± 0.20 \\
    &   &    & (b)   &       &       & \textbf{17.01 ± 9.34} & \textbf{0.15 ± 0.14} & 0.51 ± 0.20  \\
    \cmidrule{7-7}
    &   &    & (c)   & \multirow{2}[0]{*}{15/15} & \multirow{2}[0]{*}{\textbf{15/15}} & 17.16 ± 9.31 & 0.16 ± 0.17 & 0.51 ± 0.22 \\
    &   &    & (d)   &       &       & 17.09 ± 9.26 & \textbf{0.11 ± 0.10} & \textbf{0.55 ± 0.21}  \\
    \midrule
    \end{tabular}%
  \end{adjustwidth}
  \caption{Quantitative and qualitative evaluation of scene reconstruction using our ACDC method in a sim-to-sim scenario. `Scale' is the largest distance between two objects' bounding boxes in the input scene. `Cat.' indicates the ratio of correctly categorized objects to the total number of objects in the scene. `Mod.' shows the ratio of correctly modeled objects to the total number of objects in the scene. `L2 Dist' provides the mean and standard deviation of the Euclidean distance between the centers of the bounding boxes in the input and reconstructed scenes. `Ori. Diff.' represents the mean and standard deviation of the orientation magnitude difference of each non-uniformly symmetric object. `Bbox IoU' presents the Intersection over Union (IoU) for assets' 3D bounding boxes. Please refer to the supplementary material for extension of this table.\label{tab:sim2sim}}
\end{table}%
